Oracle-free Reinforcement Learning in Mean-Field Games along a Single Sample Path

We consider online reinforcement learning in Mean-Field Games (MFGs). Unlike traditional approaches, we alleviate the need for a mean-field oracle by developing an algorithm that approximates the Mean-Field Equilibrium (MFE) using the single sample path of the generic agent. We call this {\it Sandbox Learning}, as it can be used as a warm-start for any agent learning in a multi-agent non-cooperative setting. We adopt a two time-scale approach in which an online fixed-point recursion for the mean-field operates on a slower time-scale, in tandem with a control policy update on a faster time-scale for the generic agent. Given that the underlying Markov Decision Process (MDP) of the agent is communicating, we provide finite sample convergence guarantees in terms of convergence of the mean-field and control policy to the mean-field equilibrium. The sample complexity of the Sandbox learning algorithm is $\tilde{\mathcal{O}}(\epsilon^{-4})$ where $\epsilon$ is the MFE approximation error. This is similar to works which assume access to oracle. Finally, we empirically demonstrate the effectiveness of the sandbox learning algorithm in diverse scenarios, including those where the MDP does not necessarily have a single communicating class.

==> Sec_check.tex <==

% 	%%% BEGIN INSTRUCTIONS %%%
% 	The checklist follows the references.  Please
% 	read the checklist guidelines carefully for information on how to answer these
% 	questions.  For each question, change the default \answerTODO{} to \answerYes{},
% 	\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% 		justification to your answer}, either by referencing the appropriate section of
% 	your paper or providing a brief inline description.  For example:
% 	\begin{itemize}
% 		\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% 		\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% 		\item Did you include the license to the code and datasets? \answerNA{}
% 	\end{itemize}
% 	Please do not modify the questions and only use the provided macros for your
% 	answers.  Note that the Checklist section does not count towards the page
% 	limit.  In your paper, please delete this instructions block and only keep the
% 	Checklist section heading above along with the questions/answers below.
% 	%%% END INSTRUCTIONS %%%
	
	
	\begin{enumerate}
		
		
		\item For all authors...
		\begin{enumerate}
			\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
			\answerYes{}
			\item Did you describe the limitations of your work?
			\answerYes{} See Assumptions \ref{asm:contrct}--\ref{asm:act_gap} and future work for limitations.
			\item Did you discuss any potential negative societal impacts of your work?
			\answerNA{}
			\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
			\answerYes{}
		\end{enumerate}
		
		
		\item If you are including theoretical results...
		\begin{enumerate}
			\item Did you state the full set of assumptions of all theoretical results?
			\answerYes{}
			\item Did you include complete proofs of all theoretical results?
			\answerYes{} in the Supplementary Materials.
		\end{enumerate}
		
		
		\item If you ran experiments...
		\begin{enumerate}
			\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
			\answerYes{} To be included in Supplemenmtary Materials
			\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
			\answerYes{} To be included in Supplemenmtary Materials
			\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
			\answerNo{}
			\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
			\answerNA{}
		\end{enumerate}
		
		
		\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
		\begin{enumerate}
			\item If your work uses existing assets, did you cite the creators?
			\answerNA{}
			\item Did you mention the license of the assets?
			\answerNA{}
			\item Did you include any new assets either in the supplemental material or as a URL?
			\answerNA{}
			\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
			\answerNA{}
			\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
			\answerNA{}
		\end{enumerate}
		
		
		\item If you used crowdsourcing or conducted research with human subjects...
		\begin{enumerate}
			\item Did you include the full text of instructions given to participants and screenshots, if applicable?
			\answerNA{}
			\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
			\answerNA{}
			\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
			\answerNA{}
		\end{enumerate}
		
		
	\end{enumerate}
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	
	\appendix
	
	


==> proof_Lemma_1_old.tex <==
\subsection{Proof of Lemma \ref{lem:suff_exp}}
\begin{proof}
The exploration coefficients $\psi^k_t$ in policy update \eqref{eq:algorithm_iteration2} have the form,
\begin{align} \label{eq:psi_k_t}
\psi^k_t = \left\{ \begin{array}{ll}
0 & \text{if } t = 1, \\ \psi/(1 - \frac{c_\pi}{k^\theta})   & \text{if } t > 1 .
\end{array} \right.
\end{align}
for some $\psi \in (0,1-c_\pi)$ and $c_\pi$ and $\theta$ defined in Section \ref{subsec:sandbox_RL}. By definition $\psi^k_t < 1$. Notice that as $\psi^k_1 = 0$ there is no exploration noise added to the policy $\pi^k_t$ on the first timestep $t=1$ of each episode $k$, which leads to the convergence bounds (Theorem \ref{thm:conv_bound} and Corollary \ref{cor:final_bound}) being unaffected by the exploration noise. For subsequent timesteps $1 < t \leq T$, the exploration coefficient $\psi^k_t = \psi/(1 - \frac{c_\pi}{k^\theta})$ depends only on the episode $k \in [K]$ and is decreasing in $k$. This results in the sufficient exploration condition as shown below.

The proof consists of two parts, in the first part we show that under the policy update \eqref{eq:algorithm_iteration2} using learning coefficient $\psi^k_t$ \eqref{eq:psi_k_t} the probability of any action $a \in \As$ for any state $s \in \Ss$, will have a uniform lower bound $\pi^k_t(a \mid s) \geq \underline{\pi} > 0$ for all $k \in [K], 1 < t \leq T$. The fact that $\psi^k_t, 1 < t \leq T$ is increasing in $k$ and is equal to $\psi/(1 - \frac{c_\pi}{k^\theta})$ is pivotal in proving this claim. In the second step we show that using this uniform lower bound and the communicating MDP assumption (Assumption \ref{asm:comm}) we can prove sufficient exploration condition as shown in the statement of Lemma \ref{lem:suff_exp}.

To prove the lower bound $\underline\pi$ we start by proving a lower bound on $\pi^k_t(a \mid s)$ for a given episode $k$ and $1 < t \leq T$. Recalling the update \eqref{eq:algorithm_iteration2} for $1 < t \leq T$
\begin{align*}
\pi^k_{t} & = (1-c^k_{\pi,t}) \pi^k_{t-1} + c^k_{\pi,t} \bigg(\bigg(1-\frac{\psi}{1 - \frac{c_\pi}{k^\theta}}\bigg)\softmax{\lambda^k}{\cdot,Q^k_t} + \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \mathbbm{1}_{|\As|}  \bigg)
\end{align*}
where the last part on the right hand side is the uniform exploration noise. This can be written as follows,
\begin{align} \label{eq:cp_update_recur}
\pi^k_{t} & = \tilde{c}^k_{\pi,[2,t]} \pi^k_1 + \sum_{l=2}^t c^k_{\pi,[l,t]} \bigg( 1-\frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \bigg) \softmax{\lambda^k}{\cdot,Q^k_l} + \sum_{l=2}^t c^k_{\pi,[l,t]} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}}  \mathbbm{1}_{|\As|},
\end{align}
where
\begin{align*}
\tilde{c}^k_{\pi,[l,t]} = \prod_{s=l}^t (1 - c^k_{\pi,s}), \hspace{0.25cm} c^k_{\pi,[l,t]} = c^k_{\pi,l} \prod_{s=l+1}^t (1 - c^k_{\pi,s}).
\end{align*}
From the control policy update \eqref{eq:cp_update_recur} we analyze the last part of right hand side. In particular, we will prove that $\sum_{l=2}^{t+1} c^k_{\pi,[l,t+1]} \geq \sum_{l=2}^{t} c^k_{\pi,[l,t]}$ for $1 < t \leq T$. First we see,
\begin{align} \label{eq:c_k_pi_inter}
    c^k_{\pi,[l,t]} = c^k_{\pi,l} (1 - c^k_{\pi,t}) \prod_{s=l+1}^{t-1} (1 - c^k_{\pi,s}) = (1 - c^k_{\pi,t}) c^k_{\pi,[l,t-1]}
\end{align}
Using this condition we show,
\begin{align}
    \sum_{l=2}^{t+1} c^k_{\pi,[l,t+1]} & = c^k_{\pi,[t+1,t+1]} + \sum_{l=2}^{t} c^k_{\pi,[l,t+1]} \nonumber \\
    & = c^k_{\pi,t+1} + (1 - c^k_{\pi,t+1}) \sum_{l=2}^{t} c^k_{\pi,[l,t]} \nonumber \\
    & = c^k_{\pi,t+1} \bigg( 1 - \sum_{l=2}^{t} c^k_{\pi,[l,t]} \bigg) + \sum_{l=2}^{t} c^k_{\pi,[l,t]} \geq \sum_{l=2}^{t} c^k_{\pi,[l,t]} \label{eq:upper_bound_noise}
\end{align}
where the second inequality is obtained using \eqref{eq:c_k_pi_inter}. In the inequality we use the fact that $\sum_{l=2}^{t} c^k_{\pi,[l,t]} \leq 1$ for all $1 < t \leq T$ which can be shown using inductive reasoning. The base case is true since $c^k_{\pi,[2,2]} = c^k_{\pi,2} = \frac{c_\pi}{k^\theta 2^\zeta} < 1$ since $c_\pi \leq 1$ and $\zeta > 1$. Now assume $\sum_{l=2}^{t} c^k_{\pi,[l,t]} \leq 1$ then,
\begin{align*}
\sum_{l=2}^{t+1} c^k_{\pi,[l,t+1]} & = c^k_{\pi,t+1} + (1 - c^k_{\pi,t+1}) \sum_{l=2}^{t} c^k_{\pi,[l,t]} \leq c^k_{\pi,t+1} + 1 - c^k_{\pi,t+1} = 1
\end{align*}
Hence we have proved that $\sum_{l=2}^{t} c^k_{\pi,[l,t]} \geq c^k_{\pi,[2,2]} = c^k_{\pi,2}$ for all $1 < t \leq T$. Let us define $\underline\pi^k_t := \min_{a \in \As, s \in \Ss} \pi^k_t(a \mid s)$ as the lower limit on exploration noise in policy $\pi^k_t$ for $1 < t \leq T$. Using \eqref{eq:cp_update_recur} and we can deduce
\begin{align*}
    \underline\pi^k_t \geq \tilde c^k_{\pi,[2,t]} \underline\pi^k_1 + \sum_{l=2}^t c^k_{\pi,[l,t]} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \geq \tilde c^k_{\pi,[2,t]} \underline\pi^k_1 + c^k_{\pi,2} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}}
\end{align*}
for $1 < t \leq t$ where the second inequality uses $\sum_{l=2}^{t} c^k_{\pi,[l,t]} \geq c^k_{\pi,[2,2]} = c^k_{\pi,2}$ for all $1 < t \leq T$.
% Using this fact we can deduce a lower bound on the exploration noise (dependent on episode $k$) as follows,
% \begin{align*}
% \pi^k_t(a \mid s) \geq \sum_{l=2}^t c^k_{\pi,[l,t]} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \geq c^k_{\pi,2} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}}
% \end{align*}
% for $1 < t \leq t$ where the first inequality uses the last term on the right hand side of \eqref{eq:cp_update_recur} and the second inequality uses $\sum_{l=2}^{t} c^k_{\pi,[l,t]} \geq c^k_{\pi,[2,2]} = c^k_{\pi,2}$ for all $1 < t \leq T$. 
Now we convert it into a uniform lower bound independent of $k$. Now let us define a uniform lower bound dependent on $k$, $\underline\pi^k := \min_{1 < t \leq T} \underline\pi^k_t$. Using the above equation we can write 
Using \eqref{eq:algorithm_iteration2}
\begin{align*}
\pi^k_{2} & = \tilde{c}^k_{\pi,[1,2]} \pi^k_0 + \sum_{l=1}^2 c^k_{\pi,[l,2]} \bigg( 1-\frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \bigg) \softmax{\lambda^k}{\cdot,Q^k_l} + \sum_{l=2}^2 c^k_{\pi,[l,2]} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}}  \mathbbm{1}_{|\As|} \\
& = \tilde{c}^k_{\pi,[1,2]} \pi^{k-1}_T + \sum_{l=1}^2 c^k_{\pi,[l,2]} \bigg( 1-\frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \bigg) \softmax{\lambda^k}{\cdot,Q^k_l} + c^k_{\pi,2} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}}  \mathbbm{1}_{|\As|} 
\end{align*}
Using this relation and the definition of $\underline\pi^k$ we can write
\begin{align*}
\underline\pi^k \geq \tilde{c}^k_{\pi,[1,2]} \underline\pi^{k-1} + c^k_{\pi,2} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}}  
\end{align*}
This can be written down as
\begin{align} \label{eq:under_pi_k}
\underline\pi^k \geq \tilde\vartheta_{2,k} \underline\pi^1 + \sum_{l=1}^k \vartheta_{l,k} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}}, \hspace{0.1cm} \text{where} \hspace{0.1cm} \tilde\vartheta_{l,k} = \prod_{s=l}^k \tilde c^s_{\pi,[1,2]} \hspace{0.1cm} \text{and} \hspace{0.1cm} \vartheta_{l,k} = c^l_{\pi,2} \tilde\vartheta_{l+1,k}
\end{align}
Next we will show that $\sum_{l=1}^k \vartheta_{l,k} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}} \geq \vartheta_{1,1} \psi = \frac{c_{\pi} \psi}{2^\zeta}$ for all $k \in [K]$ which coupled with \eqref{eq:under_pi_k} naturally leads to the conclusion $\underline\pi^k \geq \frac{c_{\pi} \psi}{2^\zeta}$. By definition we have,
\begin{align*}
    \sum_{l=1}^k \vartheta_{l,k} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}} & = \vartheta_{k,k} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} + \sum_{l=1}^{k-1} \vartheta_{l,k} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}} \\
    & = c^k_{\pi,2} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} + \tilde c^k_{\pi,[1,2]} \sum_{l=1}^{k-1} \vartheta_{l,k-1} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}} \\
    & = c^k_{\pi,2} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} + (1-c^k_{\pi,1})(1-c^k_{\pi,2}) \sum_{l=1}^{k-1} \vartheta_{l,k-1} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}} \\
    & = c^k_{\pi,2} \bigg( \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} - \Big(1 - \frac{c_\pi}{k^\theta}\Big) \sum_{l=1}^{k-1} \vartheta_{l,k-1} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}}\bigg) + \Big(1 - \frac{c_\pi}{k^\theta} \Big) \sum_{l=1}^{k-1} \vartheta_{l,k-1} \frac{\psi}{1 - \frac{c_\pi}{l^\theta}} \\
    & \geq c^k_{\pi,2} \bigg( \psi -  \sum_{l=1}^{k-1} \vartheta_{l,k-1} \psi\bigg) + \Big(1 - \frac{c_\pi}{k^\theta} \Big) \sum_{l=1}^{k-1} \vartheta_{l,k-1} \frac{\psi}{1 - \frac{c_\pi}{k^\theta}} \\
    & = c^k_{\pi,2} \bigg( \psi -  \sum_{l=1}^{k-1} \vartheta_{l,k-1} \psi\bigg) +  \sum_{l=1}^{k-1} \vartheta_{l,k-1} \psi \\
    & \geq \sum_{l=1}^{k-1} \vartheta_{l,k-1} \psi
\end{align*}
\end{proof}
